Cyclic Prefix (CP) Jamming Against Eavesdropping Relays in OFDM Systems

Cooperative communication has been widely used to provide spatial diversity benefits for low-end user equipments, especially in ad hoc and wireless sensor networks. However, the lack of strong authentication mechanisms in these networks leaves them prone to eavesdropping relays. In this paper, we propose a secure orthogonal frequency division multiplexing (OFDM) transmission scheme, where the destination node transmits a jamming signal over the cyclic prefix (CP) duration of the received signal. Simulation results verify that as long as at least a part of the jamming signal falls to the actual data portion of the eavesdropping relay, it spreads through all the data symbols due to the fast Fourier transformation (FFT) operation, resulting in degraded interception at the eavesdropper.

==> AcronymList.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{PDCP}[PDCP]{packet data convergence protocol}
\acrodef{RATs}[RATs]{radio access technologies}
% \acrodefplural{RAT}[RAT]{radio access technologies}
\acrodef{AP}[AP]{access point}
\acrodef{MP-TCP}[MP-TCP]{Multipath transmission control protocol}
\acrodef{5QI}[5QI]{\ac{5G} \ac{QoS} identifier}
\acrodef{NSI}[NSI]{network slice instance}
\acrodef{ATSSS}[ATSSS]{access traffic steering, switching and splitting}
\acrodef{CA}[CA]{coordination area}
\acrodef{TRP}[TRP]{transmission-reception point}
\acrodef{SON}[SON]{self-organizing network}
\acrodef{V2X}[V2X]{vehicle-to-everything}
\acrodef{eMBB}[eMBB]{enhanced mobile broadband}
\acrodef{mMTC}[mMTC]{massive machine type communication}
\acrodef{uRLLC}[uRLLC]{ultra-reliable low latency communication}
\acrodef{CoMP}[CoMP]{coordinated multipoint}
\acrodef{LTE}[LTE]{Long Term Evolution}
\acrodef{LTE-A}[LTE-A]{LTE-Advanced}
\acrodef{3GPP}[3GPP]{3rd Generation Partnership Project}
\acrodef{FFR}[FFR]{fractional frequency reuse}
\acrodef{SFR}[SFR]{soft frequency reuse}
\acrodef{ICI}[ICI]{inter-cell interference}
\acrodef{ICIC}[ICIC]{inter-cell interference coordination}
\acrodef{eICIC}[eICIC]{enhanced \ac{ICIC}}
\acrodef{ABS}[ABS]{absolute blank subframe}
\acrodef{TP}[TP]{transmission point}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{eNB}[eNB]{eNodeB}
\acrodef{RAN}[RAN]{radio access network}
\acrodef{C-RAN}[C-RAN]{cloud-RAN}
\acrodef{RRH}[RRH]{remote radio head}
\acrodef{BBU}[BBU]{baseband unit}
\acrodef{CS}[CS]{coordinated scheduling}
\acrodef{CB}[CB]{coordinated beamforming}
\acrodef{JT}[JT]{joint transmission}
\acrodef{NC-JT}[NC-JT]{non-coherent \ac{JT}}
\acrodef{C-JT}[C-JT]{coherent \ac{JT}}
\acrodef{DPS}[DPS]{dynamic point selection}
\acrodef{TTI}[TTI]{transmission time interval}
\acrodef{UE}[UE]{user equipment}
\acrodef{RNTP}[RNTP]{relative narrowband transmission power}
\acrodef{eRNTP}[eRNTP]{enhanced \ac{RNTP}}
\acrodef{OI}[OI]{overload indicator}
\acrodef{HII}[HII]{high interference indicator}
\acrodef{HG}[HG]{Hermite-Gaussian}
\acrodef{CQI}[CQI]{channel quality indicator}
\acrodef{PMI}[PMI]{precoding matrix indicator}
\acrodef{RI}[RI]{rank indicator}
\acrodef{HetNet}[HetNet]{heterogeneous network}
\acrodef{mmWave}[mmWave]{millimeter wave}
\acrodef{SINR}[SINR]{signal-to-interference-plus-noise ratio}
\acrodef{SC}[SC]{single-carrier}
\acrodef{SM-OFDM}[SM-OFDM]{Spatial modulation-OFDM}
\acrodef{GB}[GB]{guard band}
\acrodef{DL}[DL]{downlink}
\acrodef{FFT}[FFT]{fast Fourier transform}
\acrodef{IFFT}[IFFT]{inverse \ac{FFT}}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{GBR}[GBR]{guaranteed bit-rate}
\acrodef{GFDM}[GFDM]{generalized orthogonal frequency division multiplexing}
\acrodef{RSRP}[RSRP]{reference signal received power}
\acrodef{CSI-RSRP}[CSI-RSRP]{CSI-reference signal received power}
\acrodef{se}[SE]{spectral efficiency}
\acrodef{5G}[5G]{fifth generation}
\acrodef{4G}[4G]{fourth generation}
\acrodef{papr}[PAPR]{peak-to-average power ratio}
\acrodef{isi}[ISI]{intersymbol interference}
\acrodef{wdm}[WDM]{waveform division multiplexing}
\acrodef{noma}[NOMA]{non-orthogonal multiple access}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{GCoMP}[GCoMP]{generalized CoMP}
\acrodef{CU}[CU]{central unit}
\acrodef{DU}[DU]{distributed unit}
\acrodef{RU}[RU]{remote unit}
\acrodef{FH}[FH]{fronthaul}
\acrodef{LoS}[LoS]{line-of-sight}
\acrodef{TBS}[TBS]{terrestrial base station}
\acrodef{FBS}[FBS]{flying base station}
\acrodef{PLS}[PLS]{physical layer security}
\acrodef{PRB}[PRB]{physical resource block}
\acrodef{PSK}[PSK]{phase-shift keying}
\acrodef{QAM}[QAM]{quadrature amplitude modulation}
\acrodef{ostbc}[OSTBC]{orthogonal space time block codes}
\acrodef{OOBE}[OOBE]{out-of-band emission}
\acrodef{svd}[SVD]{singular value decomposition}
\acrodef{MAC}[MAC]{medium access control}
\acrodef{PHY}[PHY]{physical}
\acrodef{THz}[THz]{terahertz}
\acrodef{RIS}[RIS]{reconfigurable intelligent surface}
\acrodef{QoS}[QoS]{quality of service}
\acrodef{ITS}[ITS]{intelligent transportation system}
% \acrodef{TRxP}[TRxP]{transmission reception point}
\acrodef{HO}[HO]{handover}
\acrodef{TUBITAK}[TUBITAK]{Scientific and Technological Research Council of Turkey}
\acrodef{MBB}[MBB]{\textit{Make-Before-Break}}
\acrodef{RACH}[RACH]{\textit{Random Access Channel}}
\acrodef{eMTC}[eMTC]{\textit{enhanced machine type communication}}
\acrodefplural{GBR}[GBR]{guaranteed bit rate}
\acrodef{RB}[RB]{resource block}
\acrodef{PPP}[PPP]{Poisson point process}
\acrodef{ZF}[ZF]{zero-forcing}
\acrodef{RSSI}[RSSI]{received signal strength indicator}
\acrodef{CIR}[CIR]{channel impulse response}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{ISI}[ISI]{inter-symbol interference}
\acrodef{UAV}[UAV]{unmanned aerial vehicle}
\acrodef{ISD}[ISD]{inter-site distance}
\acrodef{OFDM}[OFDM]{orthogonal frequency-division multiplexing}
\acrodef{BER}[BER]{bit error rate}
\acrodef{CSF}[CSF]{channel shortening filter}
\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{TDD}[TDD]{time division duplex}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{MSSNR}[MSSNR]{maximum shortening signal-to-noise ratio}
\acrodef{PSD}[PSD]{power spectral density}
\acrodef{QPSK}[QPSK]{Quadrature Phase Shift Keying}
\acrodef{IoT}[IoT]{Internet of Things}
\acrodef{WSN}[WSN]{wireless sensor network}
\acrodef{MRC}[MRC]{maximum-ratio combining}
\acrodef{AAF}[AAF]{amplify-and-forward}
\acrodef{CFR}[CFR]{channel frequency response}
